Smoothed Geometry for Robust Attribution

Feature attributions are a popular tool for explaining the behavior of Deep Neural Networks (DNNs), but have recently been shown to be vulnerable to attacks that produce divergent explanations for nearby inputs. This lack of robustness is especially problematic in high-stakes applications where adversarially-manipulated explanations could impair safety and trustworthiness. Building on a geometric understanding of these attacks presented in recent work, we identify Lipschitz continuity conditions on models' gradient that lead to robust gradient-based attributions, and observe that smoothness may also be related to the ability of an attack to transfer across multiple attribution methods. To mitigate these attacks in practice, we propose an inexpensive regularization method that promotes these conditions in DNNs, as well as a stochastic smoothing technique that does not require re-training. Our experiments on a range of image models demonstrate that both of these mitigations consistently improve attribution robustness, and confirm the role that smooth geometry plays in these attacks on real, large-scale models.

==> Others.tex <==
\section*{Others}

==> TRA_backup.tex <==
\section{Towards Robust Attribution}
\subsection{Bonus of Adversarial Training}
Adversarial training as a technique to increase the robustness of model's prediction augments the training data with adversarial examples \zifan{citation}. The objective can be written as
\begin{align}
\label{eq: robust prediciton}
    \min_{\boldsymbol{\theta}} \mathbb{E}_{(\mathbf{x}, y) \sim \mathcal{D}} [L((\mathbf{x}, y); \boldsymbol{\theta}) + \alpha\max_{||\boldsymbol{\epsilon}||<\delta_p}L((\mathbf{x}+\boldsymbol{\epsilon}, y)]    
\end{align} where $L$ is the training loss, e.g. Cross Entropy and $alpha$ is a hyper-parameter to control the penaty. It is intuitive to ask: \textit{will the geometry of a model with adversarial training become more smooth so that the attribution maps are more robust?} In this section, we give a theoretical analysis to approach the answer. Firstly, we denote $\Delta L = |\max_{||\boldsymbol{\epsilon}||<\delta_p}L((\mathbf{x}+\boldsymbol{\epsilon}, y) - L((\mathbf{x}, y)|$. With second-order Taylor expansion~\zifan{citation}, we can write 
\begin{align}
    \Delta L = f()
\end{align}



\subsection{An Alternative Surface Smoothing}
Users demanding robust interpretations are not always willing to afford extra budget for re-training. Except convolution with Guassian function, there is an alternative surface smoothing technique widely used in the mesh smoothing, \emph{laplacian smoothing}~\cite{Herrmann1976LaplacianIsoparametricGG, 10.1145/1057432.1057456}. The key idea behind \emph{laplacian smoothing} is that it replace the value of a point of interest on a surface using the aggregation of all neighbors within a specific distance. Adapting the motivation of \emph{laplacian smoothing}, we examine the smoothing performance of UniGrad in this paper as well.
\begin{definition}[UniGrad] Given an input point $\mathbf{x}$, the UniGrad $UG_c(\mathbf{x})$ is defined as:
$
    g(\mathbf{x}) = \triangledown_\mathbf{x}\mathbb{E}_pf_(\mathbf{z}) = \mathbb{E}_p \triangledown_\mathbf{x}f(\mathbf{z})
$ where $p(\mathbf{z}) = U(\xvec, r)$ is a uniform distribution centered at $\xvec$ with radius r.
\end{definition} 
The second equality holds since the integral boundaries are not a function of the input due to the Leibniz integral rule. One advantage of UniGrad is that, compared with SmoothGrad where more non-neighboring points may be sampled far away from the input with a higher noise level, the furthest distance of a neighboring point is controllable by $r$. In the implementation, directly sampling from a high-dimensional space with equal probability can be hard, therefore, we approximate it by sampling a uniform noise $U(x_i, r)$ for each dimension. 

